The Amazon Nova Family of Models: Technical Report and Model Card

We present Amazon Nova, a new generation of state-of-the-art foundation models that deliver frontier intelligence and industry-leading price performance. Amazon Nova Pro is a highly-capable multimodal model with the best combination of accuracy, speed, and cost for a wide range of tasks. Amazon Nova Lite is a low-cost multimodal model that is lightning fast for processing images, video, documents and text. Amazon Nova Micro is a text-only model that delivers our lowest-latency responses at very low cost. Amazon Nova Canvas is an image generation model that creates professional grade images with rich customization controls. Amazon Nova Reel is a video generation model offering high-quality outputs, customization, and motion control. Our models were built responsibly and with a commitment to customer trust, security, and reliability. We report benchmarking results for core capabilities, agentic performance, long context, functional adaptation, runtime performance, and human evaluation.

==> figures/mm_intelligence_qualitative_example_05.tex <==
\begin{mdframed}[linewidth=0.5pt,roundcorner=5pt]
    \begin{minipage}[t]{0.48\textwidth}
        \textbf{\large User input} %
        \vspace{1.5em} %

        \begin{wrapfigure}{r}{0.5\textwidth} %
            \vspace{-1.2em} %
            \includegraphics[width=0.48\textwidth]{figures/mm_intelligence_qualitative_example_05.jpg}
        \end{wrapfigure}
        
        This looks like an amazing site. What is it and where is it located? Are there other fun things around this site to explore?
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\textwidth}
        \textbf{\large Response} %
        \vspace{1.5em} %

        This is the Space Needle, a landmark in Seattle, Washington, USA. It is a well-known observation tower and a symbol of Seattle. It was built for the 1962 World's Fair and has since become a popular tourist attraction. The Space Needle offers panoramic views of the city, the surrounding mountains, and the Puget Sound.

        The Space Needle is located in the Seattle Center, which is a cultural and entertainment hub. The Seattle Center is home to many other attractions, including the Chihuly Garden and Glass, the Museum of Pop Culture, and the Pacific Science Center. The Seattle Center also hosts events like concerts, festivals, and art exhibitions.

        The Seattle Center is also close to other popular attractions in Seattle, such as the Pike Place Market, the Seattle Aquarium, and the Seattle Art Museum. The city is known for its vibrant arts and culture scene, outdoor activities, and beautiful natural surroundings.
    \end{minipage}
\end{mdframed}


